EG-VQA: Benchmarking Verifiable Video Question Answering with Grounded Temporal Evidence

Recent advances in Video Large Language Models (Video-LLMs) have yielded promising performance on Video Question Answering (VideoQA). Nevertheless, existing benchmarks are predominantly evaluated through answer correctness, while the faithfulness of predicted evidence supporting those answers remains insufficiently evaluated. This disconnect between answer generation and evidence verification motivates the construction of the Evidence-Grounded Video Question Answering Benchmark (EG-VQA), a large-scale open-ended benchmark in which each QA pair is annotated with temporally localized textual evidence, requiring models to jointly produce answers and verifiable evidence. EG-VQA comprises 2,067 videos and 11,838 QA pairs with fine-grained evidence annotations. To evaluate predicted evidence, Evidence-Grounded F1 (EG-F1) is introduced as a metric that jointly measures temporal alignment and semantic consistency between predicted and ground-truth evidence. Experiments reveal a substantial discrepancy between answer correctness and evidence faithfulness: even strong proprietary models can achieve high answer accuracy while exhibiting gaps in temporal-semantic grounding. To investigate evidence-aware learning under EG-VQA, we develop EG-Reasoner, an evidence-aware model trained with explicit evidence supervision. EG-Reasoner achieves strong evidence grounding performance among open-source models while maintaining competitive answer generation results compared with proprietary systems. These findings highlight the importance of explicitly modeling evidence grounding and suggest that evidence-aware supervision provides an effective direction toward more reliable and interpretable VideoQA systems.

==> table/benchmark_validity.tex <==
\begin{figure}[t]
\centering

\begin{minipage}[t]{0.45\columnwidth}
\vspace{0pt}
\centering
\includegraphics[width=\linewidth]{figures/answer_correctness_vs_evidence_grounding.pdf}

\vspace{-2mm}
\captionof{figure}{Comparison between answer correctness and evidence faithfulness across models.}
\label{fig:answer_evidence_comparison_iou_sensitivity}
\end{minipage}
\hspace{0.00\columnwidth}
\begin{minipage}[t]{0.53\columnwidth}
\vspace{0pt}
\centering

\scriptsize
\setlength{\tabcolsep}{2.7pt}
\renewcommand{\arraystretch}{1.6}

\begin{tabular}{llcc}
\toprule
\textbf{Model} & \textbf{Input} & \textbf{Relaxed Acc. $\uparrow$} & \textbf{Avg. EG-F1 $\uparrow$} \\
\midrule
\multirow{3}{*}{Qwen2.5-VL-7B}
& Full Video & 27.96 & 3.33\\
& Question-only &4.36&0.06\\
& Mismatched Video&1.97&0.02\\
\midrule
\multirow{3}{*}{EG-Reasoner}
& Full Video&\textbf{42.71}&\textbf{12.28}\\
& Question-only&9.61&0.22\\
& Mismatched Video&6.77&0.31\\
\bottomrule
\end{tabular}

% \vspace{-1mm}
\vspace{2pt}
\captionof{table}{Video-dependency evaluation on EG-VQA.}
\label{tab:video_dependency}

\end{minipage}
\end{figure}

